Spurious Valleys in Two-layer Neural Network Optimization Landscapes

Neural networks provide a rich class of high-dimensional, non-convex optimization problems. Despite their non-convexity, gradient-descent methods often successfully optimize these models. This has motivated a recent spur in research attempting to characterize properties of their loss surface that may explain such success. In this paper, we address this phenomenon by studying a key topological property of the loss: the presence or absence of spurious valleys, defined as connected components of sub-level sets that do not include a global minimum. Focusing on a class of two-layer neural networks defined by smooth (but generally non-linear) activation functions, we identify a notion of intrinsic dimension and show that it provides necessary and sufficient conditions for the absence of spurious valleys. More concretely, finite intrinsic dimension guarantees that for sufficiently overparametrised models no spurious valleys exist, independently of the data distribution. Conversely, infinite intrinsic dimension implies that spurious valleys do exist for certain data distributions, independently of model overparametrisation. Besides these positive and negative results, we show that, although spurious valleys may exist in general, they are confined to low risk levels and avoided with high probability on overparametrised models.

==> journal_gap.tex <==
\section{Typical Spurious Valleys and Low-Energy Barriers}\label{sec:gap}

In the previous section it was shown that whenever the
number of hidden units $p$ is below the lower intrinsic dimension, then 
one can show worst-case data distributions that yield a landscape with arbitrarily 
bad spurious valleys. 

In this section, we study the energy landscape under generic data distributions in case of homogeneous activation, and
show that, although spurious valleys may appear, they tend do so below a certain energy level,
controlled by the decay of the spectral decomposition of the kernel defined by the activation function and by the amount of parametrisation $p$. 
This phenomena is consistent with the empirical success of gradient-descent algorithms 
in conditions where $p$ is indeed below the intrinsic dimension. 

We consider 
%$L^2$-regularized 
oracle square loss functions of the form
\begin{equation}\label{eq:mse}
L(\btheta) = \E%_{(X,Y) \sim P}
\abs*{\Phi(\bX;\btheta) - Y }^2 %+ \lambda \norm*{\bu}^2
\end{equation}
for one-dimensional output two-layers NNs $\Phi(\bx;\btheta) = \bu^T \rho(\bW \bx + \bb)$, with $\btheta = (\bu, \bb, \bW) \in \mathbb{R}^p \times \mathbb{R}^p \times \mathbb{R}^{p\times n}$, $\rho$ a positively homogeneous function,  %$\rho(z) = z_+$, 
and $\bX,Y$ square integrable r.v. ($\expval\norm{\bX}^2, \expval Y^2 < \infty$). 
Notice that we can write
\begin{equation*}
L(\btheta) = \E\abs*{\Phi(\bX;\btheta) - f^*(\bX)}^2 + \E\abs*{Y - f^*(\bX)}^2 %+ \lambda \norm*{\bu}^2
\end{equation*}
for some measurable $f^*:\mathbb{R}^n\to\mathbb{R}$ such that $f^*(\bX) = \E\parq*{Y\,|\,\bX}$. In particular this implies that
\begin{equation*}
\min_{\btheta\in\Theta}L(\btheta) \geq \mathcal{R}\parr{\bX,Y} \doteq \E\abs*{Y - f^*(\bX)}^2 %+ \lambda \norm*{\bu}^2
\end{equation*}
As $p\to \infty$, the optimization problem (\ref{eq:mse}) becomes convex, a fact that is 
exploited in several recent works \cite{mei2018mean, rotskoff2018neural, chizat2018global}. 
As observed by Bach in \cite{bach2017equivalence}, the effect of having only a finite number of hidden neurons 
can be recast as obtaining a quadrature rule for the reproducing kernel associated to the activation function.
The following theorem is a direct application of Proposition 1 from \cite{bach2017equivalence}, 
and relates the quadrature error with the ability to avoid large loss barriers with high probability. 
%with the gap between local and global minima of (\ref{eq:mse})
%states that, although (bad) spurious valleys may exist, starting in a random point of the parameter space we can avoid large (loss) barriers. This fact holds for every data distributions. 
\begin{theorem}\label{theo:energy_gap}
Let $d\tau$ be the uniform distribution over the unit sphere $\mathbb{S}^n$ and consider an initial parameter $\tilde{\btheta} = (\tilde{\bu},\tilde{\bb},\tilde{\bW})$ with $(\tilde{\bw}_i,\tilde{b}_i) \sim d\tau$ sampled i.i.d. Then the following hold:
\begin{enumerate}
\item There exists a path $t\in[0,1]\mapsto \btheta_t$ such that $\btheta_0 = \tilde{\btheta}$, the function $t\in[0,1]\mapsto L(\btheta_t)$ is non-increasing, and 
$$
L(\btheta_1) \leq \mathcal{R}(\bX,Y) + \lambda \quad\text{if}\quad p \geq O\parr*{-\lambda^{-1}\log(\lambda\delta)}
$$
with probability greater or equal then $1-\delta$, for every $\lambda,\delta \in (0,1)$.
\item If $f^*$ is sufficiently regular\footnote{More precisely, if the function $f^*$ can be written as 
$f^*(\bx) = \int_\mathcal{W} g^*(\bw)\psi_\bw(\bx)\,d\tau(\bw)$ for some $g^* \in L^\infty_{d\tau}$.}, there exists a path $t\in[0,1]\mapsto \btheta_t$ such that $\btheta_0 = \tilde{\btheta}$, the function $t\in[0,1]\mapsto L(\btheta_t)$ is non-increasing, and 
$$
L(\btheta_1) \leq \mathcal{R}(\bX,Y) + O(p^{-1+\delta})
$$
with probability greater or equal then $1-e^{-O(p^\delta)}$ for every $\delta\in(0,1)$.
\end{enumerate}
\end{theorem}


% Consider the set-up where the rows of the first-layer parameter $\bW$ (i.e. the first layer neurons) live in a measurable subset $\mathcal{W} \subseteq \mathbb{R}^n$. We assume that the subset $\mathcal{W}$ is endowed with a probability measure $d\tau$ such that the continuous function 
% \begin{equation*}
% \psi : (\bw, \bx) \in \mathcal{W} \times \mathbb{R}^n \mapsto \psi_\bw(\bx) = \rho(\prodscal{\bw,\bx})     
% \end{equation*}
% belongs to $L^2(\mathcal{W}\times \mathbb{R}^n, d\tau \otimes d\mu)$, where $d\mu$ is the probability distribution of $\bX$, and such that
% \begin{enumerate}[label=\textbf{A.\arabic*}]
% \item \label{ass:1} 
% the function $f^*$ can be written as 
% \begin{equation*}
% f^*(\bx) = \int_\mathcal{W} g^*(\bw)\psi_\bw(\bx)\,d\tau(\bw)
% \end{equation*}
% for some $g^* \in L^\infty(\mathcal{W},d\tau)$.
% \end{enumerate}
% \paragraph{Setup:} Let $L(\Theta) = \E_{(X,Y) \sim P} | U \rho(W X) - Y|^2 + \lambda \| U \|_2^2$, with $U \in \R^m$, $W \in \R^{m \times n}$, $\rho$ homogeneous, 
% with $W=(w_1, \dots w_m)$ and $\| w_i \| = 1$.  
% Let $d\mu$ be the marginal density of $X$. Let $L_* = \min_\Theta L(\Theta)$. For $w \in \R^n$, we denote 
% by $\psi_w: x \mapsto \rho(\langle w, x \rangle)$, $\psi_w \in L_2(d\mu)$. 

% Assume $\rho$ is homogeneous. 
% Following \cite{bach2017equivalence}, we consider the kernel associated with the neural network architecture
% \begin{equation}\label{eq:kernel}
% k(\bx,\by) = \int_\mathcal{W} \psi_\bw(\bx) \psi_\bw(\by)\,d\tau(\bw)
% \end{equation}
% %where $d\tau$ is a base probability measure on the $n$-dimensional sphere, such as the uniform measure. 
% The above defines a continuous symmetric, positive semi-definite kernel $k$, along with $\mathbb{H}$, the RKHS associated, and the integral operator $\Sigma : L^2(\mathbb{R}^n, d\mu) \to \mathbb{H} \subseteq L^2(\mathbb{R}^n, d\mu)$ defined as
% \begin{equation*}
% f \mapsto \parr*{\Sigma f : \bx \mapsto \int_{\mathbb{R}^n} f(\by) k(\bx,\by)\,d\mu(\by)}
% \end{equation*} 
% The operator $\Sigma$ admits a spectral decomposition in $L^2(\mathbb{R}^n, d\mu)$: $\Sigma e_k = \lambda_k e_k$ for an orthonormal basis $\bra*{e_k}_{k\geq 1}$ of $L^2(\mathbb{R}^n, d\mu)$ and non-increasing sequence of 
% non-negative eigenvalues $\bra{\lambda_k}_{k\geq 1}$. 
% The following assumption avoids degenerate cases.
% \begin{enumerate}[label=\textbf{A.\arabic*},resume]
% \item The RKHS $\mathbb{H}$ is dense in $L^2(\mathbb{R}^n,d\mu)$. \label{ass:2}
% \end{enumerate}
% Note that the above assumption is equivalent to the condition $\lambda_k > 0$ for all $k\geq 1$. The expectation in \eqref{eq:kernel} provides a singular value decomposition for $\Sigma$ 
% in terms of functions in $L^2(\mathcal{W}, d\tau)$. Indeed, given $g \in L^2(\mathcal{W}, d\tau)$, the linear operator 
% $T: L^2(\mathcal{W}, d\tau) \to L^2(\mathbb{R}^n, d\mu)$ defined as
% \begin{equation*}
% g \mapsto \parr*{T g : \bx \mapsto \int_\mathcal{W} g(\bw) \psi_\bw(\bx)\,d\tau(\bw)}
% \end{equation*}
% satisfies $\Sigma = T T^*$. It follows that there exists an orthonormal basis 
% of $L^2(\mathcal{W},d\tau)$, $\bra{f_k}_{k\geq 1}$ such that $T f_k = \lambda_k^{1/2} e_k$ and therefore
% $\psi_\bw = \sum_{k=1}^\infty \lambda_k^{1/2} f_k(\bw) e_k$.
% Finally, it can be shown \cite{bach2017breaking} that in fact $\mathbb{H} = \mathrm{Im}(T)$, and 
% thus $\mathbb{H}$ consists of functions $f$ that can be written, for some $g\in L^2(\mathcal{W}, d\tau)$ as
% \begin{equation*}
% f(\bx) = \int_\mathcal{W} g(\bw) \psi_\bw(\bx) d\tau(\bw) = \prodscal{g, \psi(\cdot,\bx)}_{L^2(\mathcal{W}, d\tau)} \quad \text{for } \bx \in \mathbb{R}^n
% \end{equation*}
% For an account of these properties, we refer to \cite{bach2017equivalence}.
% whose integral representation
% $(\Sigma f)(x) = \int k(x,x') f(x') d\mu(x')$ admits a spectral decomposition in $L^2(d\mu)$:
% $\Sigma e_j = \lambda_j e_j$ for an orthonormal basis $(e_j)_j$ of $L^2(d\mu)$ and non-increasing, 
% non-negative eigenvalues $(\lambda_m)_m$. 
% The expectation in (\ref{uy1}) provides a singular value decomposition for $\Sigma$ 
% in terms of functions in $L^2(d\tau)$. Indeed, given $g \in L^2(d\tau)$, the linear operator 
% $T: L^2(d\tau) \to L^2(d\mu)$ defined as
% $$(Tg)(x) = \int_{S^{n-1}} g(w) \psi_w(x) d\tau(w)$$
% satisfies $\Sigma = T T^*$. It follows that there exists an orthonormal basis 
% of $L^2(d\tau)$ $(f_m)_m$ such that $T f_j = \lambda_j^{1/2} e_m$ and therefore
% $\psi_w = \sum_{j} \lambda_j^{1/2} f_j(w) e_j$.

% Let $\mathcal{F}$ denote the RKHS associated with $k$.  It can be shown \cite{bach2017breaking} that in fact $\mathcal{F} = Im(T)$, and 
% thus $\mathcal{F}$ consists in functions that can be written as
% $$\forall x~,~f(x) = \int_{S^{n-1}} g(w) \psi_w d\tau(w) =\langle g, \varphi(\cdot, x) \rangle_{L^2(d\tau)}~,$$
% with $\varphi(w, x) = \rho( \langle x, w, \rangle)$. 

% Let $h(x) := \E\{ Y | X=x\}$. The loss 
% $$\bar{L}(f) = \| f - h\|^2_{L^2(d\mu)}~,~f \in \mathcal{F}$$
% is convex, and assuming wlog that the eigenvalues $\lambda_i >0$ for all $i$, the loss 
% is in fact strongly convex, thus with a unique minimiser $f^* \in \mathcal{F}$. 
% Let $g^* \in L^2(d\tau)$ be such that
% \begin{equation}
% \label{uy44}
%     f^* = \int g^*(w) \psi_w d\tau(w) ~.%\text{ for } g^* \in L^2(d\tau)~.
% \end{equation} 

% Now, given an initial set of first layer weights $\bw_1, \dots, \bw_p \in \mathcal{W}$ 
% sampled i.i.d. from $d\tau$, and $\bW = [\bw_1,\dots,\bw_p]^T$, we define the empirical kernel 
% \begin{equation*}
% k_\bW(\bx,\by) = \frac{1}{p} \sum_{i=1}^p \rho(\prodscal{\bx, \bw_i}) \rho(\prodscal{\by, \bw_i})
% \end{equation*}
% which in turn defines an empirical RKHS $\mathbb{H}_\bW$. Keeping the first layer weights fixed and optimizing the second layer weights thus gives us 
% the ability to find a function $f^*_\bW \in \mathbb{H}_\bW$ that best approximates $f^*$:
% \begin{equation*}
% \norm*{ f^*_\bW - f^* }_{L^2(\mathbb{R}^n,d\mu)}  = \min_{f \in \mathbb{H}_\bW}\norm*{f - f^*}_{L^2(\mathbb{R}^n,d\mu)} \doteq R(\bW)
% %= \left \| \sum_{i=1}^m u_i \psi_{w_i} - \int g^*(w) \psi_w d\tau(w) \right \|_{L^2(d\mu)}
% \end{equation*}
% In particular $f^*_\bW = \Phi(\cdot;\btheta)$ with $\btheta = (\bu^*_\bW, \bW)$ for some $\bu^*_\bW \in \mathbb{R}^p$.
% By taking $u_k = \frac{1}{p} g^*(\bw_k)$ for $k \in [p]$ and denoting $Z(\bw):= g^*(\bw) \psi_\bw$ and by $Z$ the r.v. $Z = Z(\bv)$, for $\bv \sim d\tau$, with values in $L^2(\mathbb{R}^n,d\mu)$, it holds
% \begin{equation}\label{eq:whp_error_bound}
% R(\bW) \leq \norm[\Big]{\frac{1}{p}\sum_{k=1}^p Z(\bw_k)- \E_\tau\parq*{Z} }_{L^2(\mathbb{R}^n, d\mu)}
% \end{equation}
% Using an Hoeffding-type inequality we get the following.
% \begin{lemma}\label{lemma:whp}
% Assume  the above setup holds and that $C \doteq \sup_{\bw \in \mathcal{W}} \norm{Z(\bw)}_{L^2(\mathbb{R}^n,d\mu)} < \infty$. Then 
% \begin{equation*}
% \mathbb{P}_\tau \bra*{ R(\bW) \leq \varepsilon } \geq 1 - \mathrm{exp}\bra*{-\parr*{\varepsilon - \sqrt{v(p)}}^2 / (2 v(p))}
% \end{equation*}
% for every $\varepsilon \geq \sqrt{v(p)}$, with $v(p) = C^2 /p$.
% \end{lemma}
% \begin{proof}
% This follows immediately by applying the result in \cite{boucheron2013concentration}, Example 6.3, to the bound \eqref{eq:whp_error_bound}. 
% \end{proof}
%Applying Lemma \ref{lemma:whp} we get the following result. 

% Since the loss function $L(\theta)$ is convex in the second layer parameters $\bu$, this implies the existence with high probability (w.h.p.) of a descent path from any initial parameter $\tilde{\btheta} =(\tilde{\bu},\tilde{\bW})$ with $\tilde{\bw}_i \sim d\tau$ i.i.d. to an energy level $\tilde{L}$ satisfying
% %$$\tilde{L} - \min_{\Theta} L(\Theta) \leq \tilde{L} - \min_{f \in \mathcal{F}} \bar{L}(f) \leq \min_{\hat{f} \in \hat{\mathcal{F}}} \| \hat{f} - f^* \|^2_{L^2(d\mu)} = \Theta(\frac{1}{m})~.$$
% \begin{equation*}
% \tilde{L} \leq \mathcal{R}\parr{\bX,Y} + R(\tilde{\bW})^2 \leq \mathcal{R}\parr{\bX,Y} + O(p^{-1})
% \end{equation*}
% In the following, we consider continuous positive homogeneous activation functions $\rho$, such as Leaky ReLU's. By positive homogeneity we mean that there exists $h : (0,\infty) \to (0,\infty)$ continuous such that $h(\lambda) = \rho(\lambda x) / \rho(x)$ for every $x$ s.t. $\rho(x) \neq 0$.
%  the error in (\ref{uy2}) satisfies 
%  \begin{eqnarray}
%  \label{uy3}
%  \E_{w_1, \dots w_m} \| \hat{f} - f \|^2 &=& \E_\tau \left \| \frac{1}{m} \sum_{i \leq m} Z(w_i) - \E_\tau Z(w) \right \|^2 = \frac{1}{m} \E_\tau \| Z - \E Z \|^2 \\ \nonumber
%  &\leq& \frac{1}{m} \|f^*\|^2_\mathcal{F} \sup_w \| \psi_w \|_{L^2(d\mu)}^2  = \Theta(1/m)~.
%  \end{eqnarray}
% And using Chernoff/Hoeffding one can obtain a result with high probability using standard 
% concentration arguments of the empirical mean. 

% {\color{red} TODO: Write the concentration result in form of Theorem}
% \begin{theorem}[High probability low energy gap for homogeneous activations]\label{theorem:energy_gap}
% Let $\rho$ be a continuous positive-homogeneus activation function and $L(\btheta)$ the square loss function \eqref{eq:mse} for two-layers NNs $\Phi(\bx;\btheta) = \bu^T\rho(\bW\bx)$ with one-dimensional output ($m=1$). Let $d\tau$ be the uniform distribution over the unit sphere $\mathbb{S}^{n-1}$. If assumptions \ref{ass:1} and \ref{ass:2} hold, 
% % and $g^* \in L^\infty(\mathbb{R}, d\tau)$
% then, for any inital parameter $\tilde{\btheta} = (\tilde{\bu},\tilde{\bW})$ with $\tilde{\bw}_i \sim d\tau$ sampled i.i.d., there exists a path $t\in[0,1]\mapsto \btheta_t$ such that $\btheta_0 = \tilde{\btheta}$, the function $t\in[0,1]\mapsto L(\btheta_t)$ is non-increasing, and 
% $$
% L(\btheta_1) \leq \mathcal{R}(\bX,Y) + O(p^{-1+\delta})
% $$
% with probability greater or equal then $1-e^{-O(p^\delta)}$ for every $\delta\in(0,1)$.
% \end{theorem}
% \begin{proof}
% First, notice that, since $\psi$ is continuous and $\mathcal{W}$ is compact, then 
% \begin{align*}
% C \doteq \sup_{\bw \in \mathcal{W}} \norm{Z(\bw)}_{L^2(\mathbb{R}^n,d\mu)} \leq \norm{g^*}_{L^\infty(\mathcal{W},d\tau)} \max_{\bw \in \mathcal{W}} \norm{\psi_\bw}_{L^2(\mathbb{R}^n,d\mu)}< \infty
% \end{align*}
% Given an initial parameter parameter value $\tilde{\btheta} = (\tilde{\bu},\tilde{\bW})$ as in the statement, consider the path
% \begin{equation*}
% \btheta_t = (t\bq(\tilde{\bW}) + (1-t)\tilde{\bu},\tilde{\bW}) \quad\text{where}\quad \bq(\tilde{\bW}) = \argmin_{\bu\in\mathbb{R}^p} L(\btheta)|_{\btheta = (\bu,\tilde{\bW})}
% \end{equation*}
% By convexity of $L$, the function $t\in[0,1]\mapsto L(\btheta_t)$ is non-increasing and, by taking $\varepsilon = v(p)^{1/2} + f(p)$ in Lemma \ref{lemma:whp}, it holds that
% \begin{align*}
% L(\btheta_1) & \leq \mathcal{R}\parr{\bX,Y} + R(\tilde{\bW}) \leq \mathcal{R}\parr{\bX,Y} + \parr*{ C p^{-1/2} + f(p)}^2 \\
% & = \mathcal{R}\parr{\bX,Y} + p^{-1}\parr*{ C + p^{1/2}f(p)}^2
% \end{align*}
% with probability greater or equal than $1 - e^{-pf(p)^2/(2C^2)}$. If we choose $f(p) = p^{\delta/2-1/2}$, we get that 
% \begin{equation*}
% L(\btheta_1) \leq \mathcal{R}\parr{\bX,Y} + O(p^{-(1-\delta)}) 
% \end{equation*}
% with probability greater or equal than $1-e^{O(p^\delta)}$ for every $\delta>0$.
% \end{proof}

% This simple argument already shows that descent paths up to a energy barrier of size $O(p^{-1/2})$ 
% exist w.h.p., and this does not even require to move the first layer weights. We notice that the constant $C$ in the above proof scales at least as the input dimension $n$. The barrier rate $O(p^{-1/2})$ can be refined using the results from \citep{bach2017equivalence}, with a slightly weaker condition on the regularity of the output variable, i.e. we only require $g^* \in L^2(\mathcal{W},d\tau)$. Applying Proposition 1 from \citep{bach2017equivalence}, it holds that
% \begin{equation*}
% R(\bW) \leq 4\lambda \quad\text{if}\quad p \geq 5d(\lambda)\log(16d(\lambda) / \delta)   
% \end{equation*}
% with probability greater or equal than $1-\delta$, where 
% \begin{align*}
% d(\lambda) &= \max_{\bw \in \mathcal{W}}\expval\parq*{\varphi_\bw(\bX)((\Sigma + \lambda I)^{-1}\varphi_\bw)(\bX) } \\
% &= \max_{\bw \in \mathcal{W}} \sum_{k=1}^\infty \frac{\lambda_k}{\lambda_k + \lambda} f_k(\bw)^2 \leq \lambda^{-1}\max_{\bw \in \mathcal{W}} \sum_{k=1}^\infty \lambda_k f_k(\bw)^2 = \lambda^{-1}\max_{\bw \in \mathcal{W}}\norm{\varphi_\bw}^2_{L^2(\mathbb{R}^n,d\mu)}
% \end{align*}
% We therefore derived the following.
% \begin{theorem}[High probability low energy gap for homogeneous activations - 1]\label{theorem:energy_gap_b}
% Assume that the assumption of Theorem \ref{theorem:energy_gap} hold, with $g^*\in L^2(\mathcal{W},d\tau)$ only. Then, for any inital parameter $\tilde{\btheta} = (\tilde{\bu},\tilde{\bW})$ with $\tilde{\bw}_i \sim d\tau$ sampled i.i.d., there exists a path $t\in[0,1]\mapsto \btheta_t$ such that $\btheta_0 = \tilde{\btheta}$, the function $t\in[0,1]\mapsto L(\btheta_t)$ is non-increasing, and 
% $$
% L(\btheta_1) \leq \lambda \quad\text{if}\quad p \geq O\parr*{-\lambda^{-1}\log(\lambda/\delta)}
% $$
% with probability greater or equal then $1-\delta$, for every $\lambda,\delta \in (0,1)$.
% \end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% COMMENTS FOR FUTURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Using Proposition 1 from \cite{bach2017equivalence} with base density $q(w) = 1$, one obtains 
% a bound potentially sharper, with $d(\alpha) = \sup_w \sum_i \frac{\lambda_i}{\lambda_i + \alpha} f_i^2(w)$, 
% $m \geq C d(\alpha) \log \frac{d(\alpha)}{\delta}$ and $\| f^* - \hat{f} \|^2_{L^2(d\mu)} \leq 4 \alpha$ with 
% probability at least $1-\delta$. 
% More importantly, \cite{bach2017equivalence} also shows that the gap of size $O(1/m)$ may be 
% reduced by modifying the first layer weights as to obtain a better \emph{quadrature} rule for 
% the integral form (\ref{uy44}). 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% COMMENTS FOR FUTURE END
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The above result implies that convex optimization over the second layer is sufficient to reach a model whose error 
relative to the best possible one is inversely proportional to the hidden-layer size (up to logarithm factors). Nevertheless, in practice, this approach will generally perform worse than standard gradient-descent training, which may require less over-parametrization to give satisfying results (see for example the numerical experiments in \citep{chizat2018global}, Section 4). 
This shows the importance of understanding gradient descent dynamics on the first layer, amenable to analysis in the limit $p\to \infty$ 
using mean-field techniques \cite{rotskoff2018neural,mei2018mean} as well as optimal transport
on Wasserstein metrics \cite{chizat2018global}. Precisely quantifying how much is gained by optimizing jointly in the non-asymptotic case remains an important open question \citep{chizat2018global} left for future work. 

%  \paragraph{Idea: } We build our result along the following steps:
% \begin{enumerate}
%     \item Let $\Theta^0 = (U^0, W^0)$, with $U^0 \in \R^m$, $W^0 \in \R^{m \times n}$ the initial parameters.
%     \item We suppose first that $\psi_{w_1^0}, \dots, \psi_{w_m^0}$ are linearly independent in $L_2(d\mu)$. 
%     \item Our objective is to prove that 
%     \begin{equation}
%     \label{bla}
%         \min_U L(U, W^0) - L_* \leq g(m)~, \text{ with  } g(m) \to 0 \text{ as } m\to \infty. 
%     \end{equation}
%     Since the loss is convex in $U$, this energy level can be trivially achieved by gradient descent. 
%     \item In order to prove (\ref{bla}), we will construct an empirical version of $P$, $\hat{P}_m$, using $m$ samples. This defines 
%     the auxiliary loss $\hat{L}_m(\Theta) = \E_{(X,Y) \sim \hat{P}} | U \rho(W X) - Y|^2 + \lambda \| U \|^2$. Note that for us $\hat{P}$ 
%     is a \emph{deterministic} object, we are free to choose the sample.
%     \item For appropriate choice of $\hat{P}$, the functions $\psi_{w_1^0}, \dots, \psi_{w_m^0}$ are still linearly independent in $L_2(d\hat{\mu})$. Then we know from the proof of theorem 5, corollary 7 that 
%     $$\min_\Theta \hat{L}_m(\Theta) = \min_U \hat{L}_m(U, W^0)~.$$ 
%     However, this breaks with regularization $\lambda >0$; see remark below. 
%     \item Let's now compare the resulting optimization problems in $U$. We have two least-squares problems of the form 
%     $$l(U) = U^\top \Sigma U - 2 U^\top \gamma + \sigma^2~,$$
%     with $\Sigma = \E [\Psi_W \otimes \Psi_W] + \lambda I\in \R^{m \times m}$, $\gamma = \E [Y \Psi_W] \in \R^m$, $\sigma^2 = \E Y^2$. 
%     We denote respectively $\widehat{\Sigma}, \widehat{\gamma}$ and $\widehat{\sigma^2}$ the respective moments using $\hat{P}$ instead of $P$. 
%     \item The least-squares problem is strongly convex, and therefore the global minimum of $L(U, W^0)$ with respect to $U$ can be obtained, 
%     given explicitly by $U^* = \Sigma^{-1} \gamma$ and $\hat{U}^* = \widehat{\Sigma}^{-1} \widehat{\gamma}$.
%     For a given quadrature $\hat{P}$ we have a bound of the form $| L(U^*, W^0) - \hat{L}( \hat{U}^*, W^0)| \leq f(m)$, since 
%     we expect $\Sigma - \widehat{\Sigma}$, $\gamma - \widehat{\gamma}$ and $\sigma^2 - \widehat{\sigma^2}$ to be small as $m$ increases (subtle). 
%     \item It results that 
%     \begin{equation}
%     \label{blee}
%         | L(U^*, W^0) - \min_{\Theta} \hat{L}( \Theta) | \leq f(m). 
%     \end{equation}
%     \item Finally, using the Rademacher complexity ($W$ lives in a compact space and $U$ is penalized in norm), we have a uniform bound of the form 
%     $$| \min_\Theta L(\Theta) - \min_{\Theta} \hat{L}(\Theta) | \leq h(m)~,\text{ with } h(m) \simeq 1 / \sqrt{m} ~,$$
%     which together with (\ref{blee}) implies (\ref{bla}) with $g(m) = h(m) + f(m)$.
% \end{enumerate}


% \paragraph{Remarks:}
% \begin{itemize}
% \item This result attempts to show that, for sufficiently large $m$, optimizing the second layer weights alone brings the loss closer and closer 
% to the global optimum. How close to the global optimum depends on our ability to find a quadrature rule that approximates functions 
% on the RKHS defined by $(\rho, P)$. 

% \item The paths that only move second layer weights are `mixture' paths, whereas paths that also move first layer weights (while second layer ones are non-zero) are `transport' paths. We have seen throughout the paper that there is no generic procedure to construct transport paths, but 
% on some special cases they allow us to improve the bounds (linear and quadratic case). 

%     \item The main technical challenge is that as $m$ increases, the covariance operator we need to approximate grows, $\Sigma \in \R^{m \times m}$. 
% The quadrature rules of Bach (2017) are in the setting where the sampling is decoupled from the functions to approximate. 

% \item The case where we replace the ridge regression regularisation $\| U \|^2$ by the sparsity $\|U \|_1$ is also possible, and somewhat easier. 
% The construction of the descent path in that case is explicit, by expoiting the zeros in $U$ and filling-in the optimal first-layer weights in the corresponding locations.

% \item The result may be too strong as it is stated now, because it likely that our rate $g(m)$ in fact depends on the initial first layer 
% weights $W^0$. For `incoherent' first-layer weights, we expect it to approximate well the functions, but one could imagine adversarial 
% initializations that make this approximation very bad. If the approximation has full rank $m$, then we do not know in general how to do transports
% that do not increase the loss. 

% \item In fact, the role of regularization ($\lambda >0$) is key. If $\lambda >0$, I believe the general result of corollary 7 is false. This is somewhat a good thing, because it shows the problem is not trivial, only by mixture paths you cannot in general reach the global min. 

% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% L^1 CASE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{$\ell_1$ Case}

% In this case, the path is constructed by iterating the following procedure. 

% \begin{enumerate}
%     \item Solve the second layer weights keeping first layer fixed:
%     $$\min_{U} \| \sum_i u_i \psi_{w_i} - h \|^2_{L^2(d\mu)} + \beta \| U \|_1$$
%     This is the sparse regression (lasso) problem.
%     \item On the entries $u_i =0$, replace the corresponding $w_i$ by a better atom. 
% \end{enumerate}

% This algorithm can be visualized as visiting saddle points (since $u_i=0$ creates a saddle in the 
% corresponding coordinate $w_i$) iteratively. 

% {\color{red} TODO: 
% \begin{itemize}
%     \item check from literature the conditions (depending on empirical kernel $\hat{k}$ and
% regularization parameter $\beta$) that create zeros in $U$. 
%     \item decide how to update the $w_i$. 
%     \item Can we prove that we get a bound sharper than $1/m$ ? 
% \end{itemize}
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END L^1 CASE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> journal_intro.tex <==
\section{Introduction}\label{section:introduction}

Modern machine learning applications involve datasets of increasing dimensionality, complexity and size, which in turn motivate the use of high-dimensional, non-linear models, as illustrated in many deep learning algorithms across computer vision, speech and natural language understanding. The prevalent strategy for learning is to rely on Stochastic Gradient Descent (SGD) methods, that typically operate on non-convex objectives. In this context, an outstanding goal is to provide a theoretical framework that explains under what conditions -- relating input data distribution, choice of architecture and choice of optimization scheme -- this setup will be successful. 

More precisely, let $\bPhi_\btheta\, :\, \mathbb{R}^n \to \mathbb{R}^m$  denote a model class parametrized by $\btheta \in \Theta\subseteq  \mathbb{R}^P$, which in the case of Neural Networks (NNs) contains the aggregated weights across all layers. In a supervised learning setting, this model is deployed on some data $(\bX,\bY)$ random variable taking values in $\mathbb{R}^n\times \mathbb{R}^m$, to predict targets $\bY$ given features $\bX$, and its risk for a given $\btheta$ is 
\begin{equation}
\label{riskeq}
L(\btheta) = \mathbb{E}_{(\bX,\bY) \sim P} \parq*{\ell( \bPhi_\btheta(\bX), \bY)}
\end{equation}
where $\ell$ is a convex loss, such as a square loss or a logistic regression loss. In the following we refer to \eqref{riskeq} as the risk, the energy or the loss interchangeably. The aim is to find $ \btheta^* \in \argmin_{\btheta \in \Theta} L(\btheta)$
and this is attempted in practice by running SGD iteration on the parameter
\begin{equation*}
\btheta_{k+1} = \btheta_k - \alpha_k \nabla_\btheta |_{\btheta = \btheta_k} \frac{1}{M} \sum_{j = 1}^M \ell( \bPhi_\btheta(\bx_j), \by_j )
\end{equation*}
where $\bra{(\bx_j,\by_j)}_{j=1}^M$ are (i.i.d.) drawn from $P$.
Under some technical conditions, the expected gradient $\expval\parq*{ \nabla_\btheta |_{\btheta = \btheta_k} L(\btheta) }$ is known to converge to $\bzero$ \citep{bottou2016optimization}. Understanding the nature of such stationary points - and therefore the landscape of the loss function - is a task of fundamental importance to understand performance of SGD. 

Whereas there is a growing literature in analyzing the behavior of SGD on non-convex objectives \citep{soudry2017implicit, ji2018risk, gunasekar2018characterizing, wilson2017marginal}, 
we focus here on properties of the optimization problem above that are algorithm independent. 
Many authors in the literature have attempted to characterize the landscape of the loss function \eqref{riskeq} by studying its critical points. Global optimality results have been obtained for NN architectures with  linear activations \citep{hardt2016identity,kawaguchi2016deep,yun2018small}, quadratic activations~\citep{soltanolkotabi2017theoretical,du2018power} and some more general non-linear activations, under appropriate regularity assumptions \citep{soudry2016no,nguyen2017loss,feizi2017porcupine}. Some other insights have been obtained by leveraging tools for complexity analysis of spin glasses \citep{choromanska2015loss} and random matrix theory \citep{pennington2017geometry}.
Other analysis involved studying goodness of the initialization of the parameter values $\btheta_0$~\citep{daniely2016toward,safran2016quality,du2017gradient} or other topological properties of the loss \eqref{riskeq}, such as connectivity of sub-level sets \citep{draxler2018essentially,brunatopology}.
A common factor shared in the above cited works (and in common practice) is that \emph{overparametrisation} of the model class (i.e. $D \gg 1$) often leads to improved performance, despite the potential increase in generalization error.

Each model defines a functional space $ \mathrm{span}\parr*{ \{ \bfun = \bPhi_\btheta \st \btheta \in \Theta\}}$, whose complexity a priori increases with the dimensionality $D$ of the parameter space $\Theta$. Whereas several authors have studied these models from the lens of approximation theory \citep{cohen2016convolutional, cohen2016expressive,bolcskei2017optimal} by focusing on specific aspects of the parameterisation (such as the depth of the network), in this work we explore another hypothesis, namely that over-parameterization remedies the complexity of that functional space, often leading to loss functions $L(\btheta)$ without poor local minima. %despite their non-convexity. 

Our approach is inspired by Freeman and Bruna \citep{brunatopology}, and is related to recent work that also explores convexifications of neural networks \citep{bach2017breaking,zhang2016convexified, bietti2017group}. 
Our analysis focuses mostly on the class of one-hidden-layer neural networks, with a hidden layer of size $p$, and covers both empirical and population risk landscapes. A given activation function $\sigma$ determines a functional space $V_\sigma = \mathrm{span}\parr*{  \{ \bx \mapsto \sigma( \langle \bx, \bw \rangle ) \st  \bw \in \R^n\} }$. In essence, our work identifies 
notions of \emph{intrinsic dimension} of this functional space, and establishes the following facts: 
\begin{enumerate}
    \item If the hidden layer size $p$ is at least equal to the \emph{upper} intrinsic dimension, then the resulting loss landscape is free of poor local minima, independently of the data distribution;
\item If $p$ is smaller than the \emph{lower} intrinsic dimension, then there exist data distributions yielding arbitrarily poor local minima.
\end{enumerate}

We articulate the notion of poor local minima via what we call \emph{spurious valleys}, defined as connected components of the sublevel sets that do not contain a global minima.
Upper and lower intrinsic dimensions define only two scenarios: either (i) they are both finite, enabling positive results; or (ii) they are both infinite, implying the negative results. Moreover, case (i) only occurs for polynomial activation functions or when the data distribution is discrete, corresponding to generic empirical risk minimization. %In that case, The positive result covers the case of polynomial activations (and in particular multilinear networks), as well as generic empirical risk minimization, which generalizes and unifies previously known results. 
The negative result covers many classes of activation functions with infinite intrinsic dimension. In particular, they generalize previously known negative results (such as leaky ReLUs) \citep{yun2018small,safran2017spurious} to a far wider class of activations. 
While in general the upper and lower intrinsic dimension may not match, we show that in some cases (linear and quadratic networks) the gap between the positive and negative results can be closed by improving on the former. 

The negative results are worst-case in nature, and leave open the question of how complex is a `typical' energy landscape corresponding to a generic data distribution. We answer this question by showing that, even if spurious valleys may appear in general, they are in practice easily avoided from random initializations, up to a low energy threshold, which approaches the global minimum at a rate inversely proportional to the hidden layer size up to log factors. 
This fact is shown for networks with homogeneous activations and generic data distributions and it is based on properties of random kernel quadrature rules \citep{bach2017equivalence}.

%in line with common practice and with analogies between glassy systems in statistical physics \citep{auffinger2013random} and neural networks~\citep{choromanska2015loss}.

Many other type of analysis of the convergence of NNs gradient-based optimization algorithms have been considered in the literature. For example, \citep{ge2017learning} proved convergence of GD on a modified loss; \citep{shamir2018resnets} compared optimization properties of residual networks with respect to linear models; in  \citep{dauphin2014identifying} it is argued that the issues arising in the optimization of NN architectures are due to the presence of saddle points in the loss function rather than spurious local minima. Optimization landscapes have also been studied in other contexts than from NNs training, such as non-convex low rank problems \citep{ge2017no}, matrix completion \citep{ge2016matrix}, problems arising in semidefinite programming \citep{boumal2016non,bandeira2016low} and implicit generative modeling \citep{bottou2017geometrical}.

The rest of the paper is structured as follows. Section \ref{section:problem_setting} formally introduces the notion
of spurious valleys and explains why this is a relevant concept from the optimization point of view. It also defines the intrinsic dimensions of a network (Section \ref{sec:dimension}).  
In Section~\ref{sec:no spurious valleys} we state our main positive results (Theorem \ref{master_theorem}) and we discuss two settings where they bear fruit: polynomial activation functions and empirical risk minimization.
% For the case of linear and quadratic activations, we improve on our general result, by proving that, for the linear case, Theorem \ref{master_theorem} holds without any assumptions on the distributions of the data or on the size/rank of any variables (which extends previous results on the optimization of linear NNs \citep{kawaguchi2016deep,yun2018critical}), and by recovering, for the quadratic case, results which are in line with current literature \citep{soltanolkotabi2017theoretical,du2018power}.
For the case of linear and quadratic activations, we improve on our general result as follows. For the linear case, we prove that Theorem \ref{master_theorem} holds without any assumptions on the distributions of the data or on the size/rank of any variables (which extends previous results on the optimization of linear NNs \citep{kawaguchi2016deep,yun2018small}). For the quadratic case, we recover results which are in line with current literature \citep{soltanolkotabi2017theoretical,du2018power}.
Section \ref{sec:spurious valleys exist} is dedicated to constructions of worst case scenarios for activation with infinite lower intrinsic dimension. We then show, in Section \ref{sec:gap}, that, even if spurious valleys may exist, they tend to be confined to regimes of low risk.  
Some discussion is reported in Section \ref{section:discussion}.

\subsection{Notation}\label{sec:notation}

We introduce notation we use throughout the rest of the paper.
For any integers $n\leq m$ we denote $[n,m] = \bra{n,n+1,\dots,m}$ and, if $n >0$, $[n] = [1,n]$.
We denote scalar valued variables as lowercase non-bold; vector valued variables as lowercase bold; matrix and tensor valued variables and multivariate random variables (r.v.'s) as uppercase bold. Given a vector $\bv\in\mathbb{R}^n$, we denote its components as $v_i$; given a matrix $\bW\in\mathbb{R}^{n\times m}$, we denote its rows as $\bw_i$;  given a tensor $\bT\in\mathbb{R}^{n_1\times \cdots \times n_k}$, we denote its components as $T_{i_1\cdots i_k}$. Given some vectors $\bv_i \in \mathbb{R}^{n_i}$, $i\in[k]$, the tensor product $\bv_1\otimes \cdots \otimes \bv_k$ denotes the $n_1\times \cdots \times n_k$ dimensional tensor $\bT$ whose components are given by $T_{i_1\cdots i_k} = v_{i_1}\cdots v_{i_k}$; given a vector $\bv$, we denote $\bv ^{\otimes k} = \otimes_{i=1}^k \bv$. We denote by $\mathrm{S}^{k}\parr*{\mathbb{R}^{n}}$ the space of order $k$ symmetric tensors on $\mathbb{R}^n$. 
For any $\bT \in \mathrm{S}^{k}\parr*{\mathbb{R}^{n}}$, we define the symmetric rank \citep{comon2008symmetric} as %$\rk_\mathrm{S}(\bT) = \min\bra*{ p \geq 1 : \bT = \sum_{i=1}^p u_i\bw_i^{\otimes k} \text{ for some }  \bw_1,\dots,\bw_p \in \mathbb{R}^n, \bu \in\mathbb{R}^p}$.
$\rk_\mathrm{S}(\bT) = \min\bra*{ p \geq 1 \st \bT = \sum_{i=1}^p u_i\bw_i^{\otimes k}\text{ for some }\bu\in\mathbb{R}^p,\bw_1,\dots,\bw_p\in\mathbb{R}^n}$.
We define $\rk_\mathrm{S}(k,n) = \max\bra{ \rk_\mathrm{S}(\bT) \st \bT \in \mathrm{S}^k(\mathbb{R}^n) }$.
Finally, $\mathbb{S}^{n-1}\subset \mathbb{R}^n$ denotes the $(n-1)$-dimensional sphere $\bra*{\bx\in\mathbb{R}^n\st \norm{\bx}=1}$.
% We say that a tensor $\bT \in \mathrm{S}^{k}\parr*{\mathbb{R}^{n}}$ is Positive Semi-Definite (PSD) if 
% %$\prodscal{\bT,\bx^{\otimes k}}_F \geq 0$ for all $\bx \in\mathbb{R}^n$. 
% there exists $\bv_1,\dots,\bv_p \in \mathbb{R}^n$ such that $\bT = \sum_{j=1}^p \bv_j^{\otimes k}$ for some $p \geq 1$\footnote{Note that this definition corresponds to the classic definition of positive semi-definiteness for the case of symmetric matrices $(k=2)$}.
% We denote by $\mathrm{S}^{k}_+\parr*{\mathbb{R}^{n}}$ the space of order $k$ PSD symmetric tensors on $\mathbb{R}^n$.

% The rest of the paper is structured as follows. Section \ref{problem_setting} formally introduces the notions 
% of spurious valleys and explains why this is a relevant property from the optimization point of view. It also defines the intrinsic dimensions of a network.  
% In Section \ref{sec:no spurious valleys} we state our main positive results (Theorem \ref{master_theorem}) and we discuss two settings where they bear fruit: polynomial activation functions and empirical risk minimization. 
% For the case of linear and quadratic activations, we improve on our general result, by extending, for the linear case, the results of \citep{kawaguchi2016deep,yun2018critical} about the optimization of linear NNs, since we can prove that Theorem \ref{master_theorem} holds without any assumptions on the distributions of the data or on the size/rank of any variables, and by recovering, for the quadratic case, results which are in line with recent works for this case \citep{soltanolkotabi2017theoretical,du2018power}. 
% Section \ref{sec:spurious valleys exist} is dedicated to constructions of worst-case scenarios for activation with infinite lower intrinsic dimension.
% Some conclusive discussion are reported in Section \ref{conclusion_section}. 

==> journal_no_valleys.tex <==
\section{Finite network dimension and absence of spurious valleys}\label{sec:no spurious valleys}

In this section we provide our positive results. Essentially they state that if the width of the network matches the dimension of the functional space $V_\rho$ spanned by its filter functions, then no spurious valleys exist. We first provide the main result (Theorem \ref{master_theorem}) in a general form, which allows a straight-forward derivation of two cases of interest: empirical risk minimization (Corollary \ref{cor:erm}) and polynomial activations (Corollary \ref{cor:poly}).  

\begin{theorem}\label{master_theorem}
For any continuous activation function $\rho$ and r.v. $\bX\in \mathcal{R}_2(\rho,n)$ with finite upper intrinsic dimension $\mathrm{dim}^*(\rho,\bX)<\infty$, the loss function $$L(\btheta) = \expval\parq*{\ell\parr*{\bPhi(\bX;\btheta),\bY}}$$
for two-layers NNs $\bPhi(\bx;\btheta) = \bU\rho( \bW\bx)$ admits no spurious valleys in the over-parametrized regime $p\geq \mathrm{dim}^*(\rho,\bX)$.
\end{theorem}
The above result can be re-phrased as follows: if the network is such that any of its output units $\Phi_i$ can be chosen from the whole linear space spanned by its filter functions $V_\rho$, then the associated optimization problem is such that there always exists a descent path to an optimal solution, for any initialization of the parameters.

Applying the observations in Section \ref{sec:dimension} describing the cases of finite intrinsic dimension, we immediately get the following corollaries.

\begin{corollary}[ERM]\label{cor:erm}
Consider $N$ data points $\bra{(\bx_i,\by_i)}_{i=1}^N \subset \mathbb{R}^{n\times m}$. For two-layers NNs $\bPhi(\bx;\btheta) = \bU\rho(\bW\bx)$, where $\rho$ is any continuous activation function, the empirical loss function 
\begin{equation*}
L(\btheta) =\frac{1}{N} \sum_{i=1}^N \ell\parr*{\bPhi(\bx_i;\btheta),\by_i}    
\end{equation*}
admits no spurious valleys in the over-parametrized regime $p \geq N$.
\end{corollary}
% \begin{proof}
% Let $\rho:\mathbb{R}\to\mathbb{R}$ a continuous activation function and $\bX$ r.v. taking (up to) $N$ values $\bx_1,\dots,\bx_N \in \mathbb{R}^n$. Since every function $f \in L^2_\bX$ is uniquely determined by the values $f(\bx_1),\dots,f(\bx_N)$ it follows that $\mathrm{dim}^*(\rho,\bX) \leq \mathrm{dim}(L^2_\bX) \leq N$. The proof is concluded by applying Theorem \ref{master_theorem}.
% \end{proof}

This result is in line with previous works that considered the landscape of empirical risk minimization for half-rectified deep networks \citep{soudry2016no,xie2016diverse,livni2014computational,nguyen2017loss}. However,
its proof illustrates the danger of studying empirical risk minimization landscapes in over-parametrized regimes, since it bypasses all the geometric and algebraic properties needed in the population risk setting - which may be more relevant to understand the generalization properties of the model.

\begin{corollary}[Polynomial activations]\label{cor:poly}
For two-layers NNs $\bPhi(\bx;\btheta) = \bU\rho(\bW\bx)$ with polynomial activation function $\rho(z) = a_0 + a_1z + \cdots + a_dz^d$, the loss function $L(\btheta) = \expval\parq*{\ell\parr*{\bPhi(\bX;\btheta),\bY}}$ admits no spurious valleys in the over-parametrized regime 
$$
p\geq \sum_{i=1}^d\binom{n + i -1}{i}\mathbf{1}_{\bra{a_i\neq 0}} = O(n^d)
$$
\end{corollary}
% \begin{proof}
% Let $\rho(z) = a_0 + a_1 z +\dots + a_dz^d$ and $\bX \sim N(\bzero,\bI)$ a standard normal r.v. with values in $\mathbb{R}^n$. Notice that $\mathrm{dim}^*(\rho,n) = \mathrm{dim}^*(\rho,\bX)$. Then, we want to show that the dimension of the vector space $V_{\rho,\bX}$
% is given by $\sum_{i=1}^d \binom{n+i -1}{i} \mathbbm{1}_{\bra{a_i \neq 0}}$. The space $V_{\rho,\bX}$ can be seen as a finite-dimensional RKHS. Consider the Gaussian RKHS $\mathbb{H}$, i.e. the one associated to the kernel
% \begin{equation*}
% \mathcal{K}:(\bx,\by)\in\mathbb{R}^n\times\mathbb{R}^n \mapsto e^{-\norm{\bx-\by}^2}
% \end{equation*}
% It is well known (see, e.g. Steinwart and Christmann \citep{steinwart2008support}) that $\mathbb{H}\simeq l^2(\mathbb{N})$ with feature map $\varphi : \mathbb{R}^n \to l^2(\mathbb{N})$: the $(k_1,\dots,k_j)$-th coordinate of $\varphi(\bx)$, where $j\in\mathbb{N}$ and $k_1,\dots,k_j\in[1,n]$, is defined as $e^{-1}(2^j/j!)^{1/2}\,x_{k_1}\cdots x_{k_j}$. Let $J = \bra{j \in [n] \st a_j \neq 0}$. We  define the map $\bw\in\mathbb{R}^n\mapsto \psi_{\rho,\bw}\in l^2(\mathbb{N})$ as follow: the the $(k_1,\dots,k_j)$-th coordinate of $\psi_{\rho,\bw}$ is $0$ if $j\notin J$ and is equal to $a_je\,(2^j/j!)^{-1/2}\,w_{k_1}\cdots w_{k_j}$ if $j \in J$. By this definition, it holds
% \begin{equation*}
% \prodscal{\psi_{\rho,\bw},\varphi(\bx)}_\mathbb{H} = \sum_{j=0}^da_j\sum_{k_1,\dots,k_j = 1}^n w_{k_1}\cdots w_{k_j}x_{k_1}\cdots x_{k_j} = \rho(\prodscal{\bw,\bx})
% \end{equation*}
% Therefore $V_{\rho,\bX}$ coincides with the linear sub-space of $\mathbb{H}$ of zero $(k_1,\dots,k_j)$-th coordinate for $j\notin J$ elements. In particular this implies that
% \begin{equation*}
% \mathrm{dim}(V_{\rho,\bX}) = \sum_{k\in J} \binom{n + k - 1}{k}
% \end{equation*}
% The proof is concluded by applying Theorem \ref{master_theorem}.
% \end{proof}
Under the hypothesis of Corollary \ref{cor:poly} with $p = O(n^d)$, a generic function of $V_\rho$, $\bPhi(\bx;\btheta) = \bu^T\rho(\bW \bx)$, can be also represented, for some $\bgamma = \bgamma(\btheta)$, in the generalized linear form 
$$
\bPhi(\bx;\btheta) = \prodscal{\bgamma, \bvarphi(\bx)}
$$
with $\bvarphi(\bx) = (x_{k_1}\cdots x_{k_j})_{\bra{1\leq k_1\leq \dots \leq k_j \leq n, j \in [d]}}$. The parameters $\btheta$ and $\bgamma$ differ for their dimensions:
$$
\dim(\bgamma) = O(n^d) < \dim(\btheta) = (n+1) \cdot O(n^d) = O(n^{d+1})
$$
One would therefore like Corollary \ref{cor:poly} to hold also (at least) for $p \geq O(n^d)$. In the next section we address this problem for the linear activation $\rho(z) = z$ and the quadratic activation $\rho(z) = z^2$.

% \begin{remark}
% From the proof of Theorem \ref{master_theorem}, it also follows that, for any initial parameter value $\tilde{\btheta} = (\tilde{\bU},\tilde{\bW})$ with $\tilde{\bw}_i$ sampled i.i.d. from a standard Gaussian distribution, for $i \in [p]$, (or, in general, from any probability distribution absolutely continuous with respect to the Lebesgue measure), then property \ref{p:conn} holds a.s. with the mapping $t\in[0,1] \mapsto L(\btheta_t)$ strictly decreasing.
% \end{remark}

\subsection{Improved over-parametrization bounds for homogeneous polynomial activations}

The over-parametrization bounds obtained in Corollary \ref{cor:poly} are quite non-desiderable in practical applications. We show that they can indeed be improved, for the case of linear and quadratic networks. 

\subsubsection{Linear networks case}

Linear networks have been considered as a first order approximation of feed-forward multi-layers networks \citep{kawaguchi2016deep}. It was shown, in several works \citep{kawaguchi2016deep,brunatopology,yun2018critical}, that, for linear networks of any depth
\begin{equation}\label{linear_NN_any_depth}
    \bPhi(\bx;\btheta) = \bW_{K+1}\cdots \bW_1 \bx
\end{equation}
with $\btheta = (\bW_{K+1},\bW_K,\dots,\bW_2,\bW_1)\in \mathbb{R}^{m\times p_{K}}\times \mathbb{R}^{p_{K}\times p_{K-1}}\times\cdots \mathbb{R}^{p_2\times p_1}\times \mathbb{R}^{p_1\times n}$, the loss function $\eqref{eq:lossFun}$ has no spurious local minima, if $\min_{i\in[K]} p_i \geq \min\bra{n,m}$. This corresponds exactly with over-parametrization regime in Corollary \ref{cor:poly}, for the case of two-layers networks. The following theorem improves on Corollary \ref{cor:poly} for the case of multi-layers linear networks, showing that no over-parametrization is required in this case to avoid spurious valleys, for square loss functions.
\begin{theorem}[Linear networks]
\label{theo:linear}
For linear NNs \eqref{linear_NN_any_depth} of any depth $K\geq 1$ and of any layer widths $p_k \geq 1$, $k\in[K]$, and any input-output dimensions $n, m \geq 1$, the square loss function $L(\btheta) = \expval\norm*{\bPhi(\bX;\btheta)-\bY}^2$ admits no spurious valleys. 
\end{theorem}

\subsubsection{Quadratic networks case}

Quadratic activations have been considered in the literature \citep{livni2014computational,du2018power,soltanolkotabi2017theoretical} as second order approximation of general non-linear activations. In particular, for two-layers networks with one dimensional output and square loss functions evaluated on $N$ samples, it was shown in  \citep{du2018power} that, if $p \geq \sqrt{2N}$, the loss has no spurious local minima. Corollary \ref{cor:poly} requires an over-parametrization bound $p \geq n(n+1)/2$ for the case of quadratic activations. In the following theorem we show that $p > 2n$ is sufficient for the statement to hold, in the case of square loss functions and one dimensional output ($m=1$).

\begin{theorem}[Quadratic networks]\label{theo:quadratic_p_geq_n}
For two-layers NNs $\Phi(\bx;\btheta) = \bu^T\rho(\bW\bx)$ with quadratic activation function $\rho(z) = z^2$ and one-dimensional output ($m=1$), the square loss function $L(\btheta) = \expval\abs*{\Phi(\bX;\btheta) - Y}^2$ admits no spurious valleys in the over-parametrized regime $p \geq 2n+1 = O(n)$. 
\end{theorem}
This result is in line with the one from  Soltanolkotabi et al.  \cite{soltanolkotabi2017theoretical}, where the authors proved absence of spurious local minima when $p\geq 2n$, but for fixed second layer weights. The proof (reported in Section \ref{sec:no spurious valleys proofs}) consists in constructing a path satisfying \ref{p:conn} and improves upon the proof of Theorem \ref{master_theorem} by leveraging the special linearized structure of the network for quadratic activation. For every parameter $\btheta = (\bu,\bW) \in \mathbb{R}^{p}\times \mathbb{R}^{p\times n}$, we can write
$$
\Phi(\bx;\btheta) = \sum_{i=1}^p u_i (\prodscal{\bw_i,\bx})^2 = \prodscal[\Big]{\sum_{i=1}^p u_i\bw_i\bw_i^T,\bx\bx^T}_F 
$$
We notice that $\Phi(\cdot;\btheta)$ can also be represented by a NN $\Phi(\cdot;\hat{\btheta})$ with 
$n$ layers; indeed, if $\sum_{i=1}^n \sigma_i \bv_i\bv_i^T$ is the SVD of $\sum_{i=1}^p u_i\bw_i\bw_i^T$, then $\Phi(\bx;\btheta) = \prodscal{\sum_{i=1}^n \sigma_i \bv_i\bv_i^T,\bx\bx^T}_F$. 
Therefore $p\geq n$ is sufficient to describe any element in $V_\rho$. The factor $2$ in the statement is due to some technicalities in the proof, but a more involved proof should be able to extend the result to the regime $p\geq n$. The extension of such mechanism for higher order tensors (appearing as a result of multiple layers or high-order polynomial activations) using tensor decomposition also seems possible and is left for future work.

\subsubsection{Lower to upper intrinsic dimension gap}

As observed in Lemma \ref{lemma:lid} $\dim_*(\rho(z)=z,n) = 1$ and $\dim_*(\rho(z)=z^2,n) = n$ for all integer $n\geq 1$. Therefore, Theorem \ref{theo:linear} and Theorem \ref{theo:quadratic_p_geq_n} say that, for $\rho(z) = z^k$, $k \in [2]$, and $m=1$, the square loss function $L(\btheta) = \expval\abs*{\Phi(\bX;\btheta) - Y}^2$ admits no spurious valleys in the over-parametrized regime $p \geq O(\dim_*(\rho,n))$. We conjecture that this hold for any (sufficiently regular) activation function with finite intrinsic lower dimension.



==> journal_related_work.tex <==
\section{Related works}\label{section:related_works}

The optimization landscape of NNs has been studied in several works, using different approaches and assumptions, both from the theoretical and empirical point of view.

Many results have been obtained from the Hessian analysis of the loss function. 
For the case of linear networks, it was shown in \citep{kawaguchi2016deep,yun2018critical} that the empirical loss function has no spurious local minima, for full-rank data covariance matrices or over-parametrized architectures. Recently, it was also shown in \citep{shamir2018resnets} that the loss functions of residual networks contains no local minima with value above what can be obtained with a linear predictor. 
Other works considered the optimization landscape of the empirical loss function of two-layers NNs with quadratic activation \citep{soltanolkotabi2017theoretical,du2018power}, which can be seen as a second order approximation of generic non-linear activation functions. Global optimality results have been recovered for quadratic networks, under sufficient over-parametrization.
The authors of \citep{nguyen2017loss} showed that, under sufficient over-parametrization, the empirical loss function of NNs of any depth with sufficiently regular activation functions is such that full-rank critical parameter values are global minima.

Many other tecniques have been explored as well.
The authors of \citep{pennington2017geometry} studied the spectral distribution of the Hessian matrix of the loss function of NNs, leveraging tools from free probability and random matrix theory.
In \citep{choromanska2015loss}, the optimization landscape of multi-layers ReLU networks has been related to spherical spin glasses \citep{auffinger2013random}.  
In \citep{dauphin2014identifying} it was argued that difficulties in optimization of NNs arises from the proliferation of saddle points rather than spurious local minima.


Other authors focused on designing a different loss function \citep{ge2017learning} with nice optimization properties, for two-layers NNs with some polynomial activation functions. 
By writing the networks in a linear fashion, the authors of \citep{soudry2016no} showed that, for almost all ReLU activation functions and input data sets, all differentiable stationary points of the empirical loss function of two-layer networks are global minima, under sufficient over-parametrization. In \citep{feizi2017porcupine}, the authors studied the case of porcupine NNs, where an incoming weight vector to a neuron is constrained to lie over a fixed line: global optimality results were recovered for ReLU two-layers NNs  and Gaussian input data, under some modeling assumptions. Goodness of random initialization of the parameter values has been studied in \citep{daniely2016toward} for general networks architectures.

Topological properties of the loss function were studied in \citep{brunatopology}: here the absence of spurious local minima is proved by showing path-connectivity of sub-level sets of the loss function, for over-parametrized linear networks and, asympotically, for ReLU two-layers NNs. The same topological property was also studied empirically in \citep{draxler2018essentially}. 
On a similar line of work, the authors of \citep{safran2016quality} introduced the concept of \emph{basin}, defined as a convex subset of the parameter space on which the sub-level sets of the loss are connected: they showed that, for ReLU two-layers NNs, the probability of initializing the parameters in a basin over which any minima of the loss function is global increases exponentially with the size of the hidden layer of the network.  

On top of the cited global optimality results, many authors provided negative results for the optimization of NNs. Hardness results for learning neural network architectures were proved in \citep{livni2014computational} and more recently in \citep{mondelli2018connection}. Global optimality has been shown to not hold in general, even for empirical loss functions evaluated on \emph{small} data sets, for non-linear architectures used in practice \citep{yun2018critical,safran2017spurious}.
